InfoVAE: Information Maximizing Variational Autoencoders

A key advance in learning generative models is the use of amortized inference distributions that are jointly trained with the models. We find that existing training objectives for variational autoencoders can lead to inaccurate amortized inference distributions and, in some cases, improving the objective provably degrades the inference quality. In addition, it has been observed that variational autoencoders tend to ignore the latent variables when combined with a decoding distribution that is too flexible. We again identify the cause in existing training criteria and propose a new class of objectives (InfoVAE) that mitigate these problems. We show that our model can significantly improve the quality of the variational posterior and can make effective use of the latent features regardless of the flexibility of the decoding distribution. Through extensive qualitative and quantitative analyses, we demonstrate that our models outperform competing approaches on multiple performance metrics.

==> prob_autoencoder.tex <==
\section{Probabilistic Autoencoder}
%\se{unregularized doesn't sound good - find a better name}
In this section, we will show that the information preference problem is caused by the regularization term $KL(q(z|x)||p(z))$, and is specific to the ELBO objective. In fact if we remove the regularization term, that is, we optimize only over the reconstruction error term in the ELBO objective,
\begin{align*}
\mathcal{L}_{AE} = E_{q_\phi(z, x)}[\log p_\theta(x|z)], \numberthis \label{equ:autoencoder}
\end{align*}
the model will prefer to maximize mutual information between $x$ and $z$. Furthermore we can still learn the data distribution $p_{data}$ and sample from the model using a Markov chain, as shown in the following Proposition~\ref{prop:unreg_vae_property}.

% \se{explain why you can't do ancestral sampling somewhere}

%\shengjia{Also run experiments on reduced regularization and show that even with a small coefficient the model still minimizes mutual information, and explain that annealing the regularization does not solve the problem}

\begin{prop}
\label{prop:unreg_vae_property}
For any $q_\phi$, if $\mathcal{L}_{AE}$ is optimized over $\theta$ for sufficiently large distribution families $\lbrace p_\theta, \theta \in \Theta \rbrace$, then
\begin{enumerate}
\item The following Markov chain converges to $p_{data}(x)$ if it is ergodic.
\begin{equation} 
\label{eq:mc}
x^{(t+1)} \sim p_\theta(x|z^{(t)}), \quad z^{(t)} \sim q_\phi(z|x^{(t)}) 
\end{equation}
\item $\mathcal{L}_{AE} = I_{q_\phi}(x; z) - H_{p_{data}}(x)$, where $I_{q_\phi}$ is mutual information under $q_\phi$ and $H_{p_{data}}$ is entropy under $p_{data}$.
\end{enumerate}
\end{prop}
\se{make this more formal. sufficiently flexible. or call it informal statement and put a formal one in appendix}

The proof is provided in the Appendix. According to Proposition~\ref{prop:unreg_vae_property}, for any $q_\phi$ the optimal value of $\mathcal{L}_{AE}$ over $\theta$ satisfies $\mathcal{L}_{AE} \propto I_{q_\phi}(x, z)$, which means that if we optimize $\mathcal{L}_{AE}$ over $\theta$ and $\phi$ jointly, it will maximize $I_{q_\phi}(x, z)$. We gain this desirable property by giving up the ability to sample ancestrally from the model. That is, $p(z)p_\theta(x|z)$ is no longer a correct generative model for $p_{data}(x)$. However we can still sample from $p_{data}(x)$ using the Markov chain described in Proposition \ref{prop:unreg_vae_property}.

A similar model from the perspective of denoising autoencoders has been proposed in \citep{dae_as_score_matching2013,dae_distribution_learning2014} and from the perspective of modeling properties of human visual learning in \citep{early_visual_concept_learning2016}. However this paper makes two novel observations, which demonstrate that these models are preferable in certain scenarios compared to ELBO autoencoders.

\textbf{1)} Probabilistic autoencoders prefer to maximize mutual information, making them useful when we need to learn features for downstream tasks such as semi-supervised learning. Note this is different from the warm-up strategy proposed in \citep{ladder_variational_network2015,nlp_vae2015}, which reduces the regularization term only initially. We observe that the warm-up strategy allows for easier optimization, but does \textbf{not} avoid the information preference problem. The mutual information drops whenever we increase the weight of the regularization term, regardless of the stage of optimization we are in.

\textbf{2)} We demonstrate empirically that samples from the model are on par with, if not superior to, a VAE trained on the ELBO criterion (ELBO-VAE) with identical architecture. The Markov chain in Proposition~\ref{prop:unreg_vae_property}  also converges reasonably fast.

%This means that if our goal is feature learning or drawing novel samples, then unregularized VAE should be a more preferable alternative to ELBO. We shall demonstrate these properties experimentally in the next section.

\subsection{Experiments}
We illustrate this on a model that uses PixelCNN \citep{pixelcnn_pp2017, pixel_rnn2015, conditional_pixelcnn2016, pixel_vae2016} as $p_\theta(x|z)$. More details on the architectures, hyper-parameters and experimental setting are provided in the appendix. 

The results are shown in Figure~\ref{fig:pixel_vae_mnist} and Figure~\ref{fig:pixel_vae_cifar}. On both MNIST and CIFAR, we can generate high quality samples (middle column) with or without regularization using the Markov chain (\ref{eq:mc}). As expected, only ELBO VAE produces high quality samples (left column) with ancestral sampling $p(z)p_\theta(x|z)$. However, the mutual information $I_q(x; z)$ between data and latent code is minimized with the ELBO criterion as shown in the top-right plot in Figure~\ref{fig:pixel_vae_mnist} and \ref{fig:pixel_vae_cifar}. In fact, mutual information is driven to zero in Figure~\ref{fig:pixel_vae_mnist} (green line), indicating that the latent code is completely ignored. On the other hand, using the $\mathcal{L}_{AE}$ objective we achieve high mutual information, as shown in the bottom-right plot of Figure~\ref{fig:pixel_vae_mnist} and \ref{fig:pixel_vae_cifar}. 

In addition, we also show that the latent features learned using the $\mathcal{L}_{AE}$ objective are useful for semi-supervised learning. The results are shown in Figure~\ref{fig:numerical_results}(E). ELBO completely fails in this task and performs no better than random guessing (as expected, given that the mutual information with the data is close to zero), while the $\mathcal{L}_{AE}$ objective achieves good semi-supervised performance, and compares favorably to all regularized methods considered in this paper.

\begin{figure*}[h]
\centering
\begin{tabular}{ccc}
\includegraphics[height=0.15\linewidth]{plot/pixel_cnn_elbo} & 
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_mnist_mc_elbo} & 
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_mnist_loss_elbo} \\ 
\includegraphics[height=0.15\linewidth]{plot/pixel_cnn_noreg} &
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_mnist_mc_noreg} & 
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_mnist_loss_noreg}
\end{tabular}
\caption{Mutual information vs sample quality for VAE with PixelCNN as family $\mathcal{P}$. \textbf{Top row}: Pixel VAE optimized on ELBO bound. \textbf{Bottom row}: Pixel VAE optimized without regularization. \textbf{Left Column}: Ancestral Samples. \textbf{Middle Column}: Markov chain samples. \textbf{Right Column}: Plot of estimated mutual information and log likelihood. For ELBO ancestral sampling $p(z)p_\theta(x|z)$ produces similar quality samples as Markov chain. For probabilistic autoencoders ancestral sampling produces nonsensical samples with ancestral sampling, while Markov chain produces samples of similar quality as ELBO. Right: evolution of estimated mutual information and per-pixel negative log likelihood loss. For ELBO, mutual information is driven to zero, indicating unused latent code, while without regularization large mutual information is preferred. Details on the mutual information computation are in the Appendix.
}
\label{fig:pixel_vae_mnist}
\end{figure*}

\begin{figure*}[h]
\centering
\begin{tabular}{ccc}
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_cifar_elbo2} &
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_cifar_mc_elbo} & 
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_cifar_loss_elbo} \\
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_cifar_noreg} &
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_cifar_mc_noreg} & 
\includegraphics[height=0.15\linewidth]{plot/pixel_vae_cifar_loss_noreg}
\end{tabular}
\caption{Experiment on CIFAR with PixelCNN. The meaning of the plots is identical to Figure~\ref{fig:pixel_vae_mnist}. The only difference is that CIFAR is too complex for our PixelCNN model to directly model the data, so the latent code is used in both cases. In both cases the mutual information is too 
%big ($\geq 14$ bits) 
difficult to directly estimate. Therefore we plot $KL(q(z|x)||p(z))$ instead.}
\label{fig:pixel_vae_cifar}
\end{figure*}


